Zeva: In-Context Causal Learning for Generalizable Embodied Manipulation

Generalizable embodied manipulation remains difficult to achieve through pretraining alone, due to unseen physical conditions in the real world. We argue that robots need to learn from their own physical interactions on the fly during real-world deployment and use this knowledge to inform subsequent actions. We present Zeva, the first framework that enables in-context learning from a robot's own physical interaction experience while keeping the policy model frozen. Zeva employs a Causal Interaction Extractor to encode an executed action and its induced state change into a causal interaction signal, which is stored in a dual-timescale causal memory. For subsequent actions, relevant causal interaction signals are retrieved from memory and injected into the frozen policy model as context. Experiments in simulation and real-world manipulation demonstrate that Zeva achieves the best performance among the compared frontier VLAs and WAMs and, more importantly, enables self-evolution during deployment without gradient updates. Its success rate continues to improve as the robot accumulates interaction experience. Furthermore, the acquired interaction experience can generalize across tasks.

==> intro-backup.tex <==
In recent years, robotics has largely followed the trajectory of large language models: knowledge is fixed into model parameters through large-scale pretraining, giving rise to a family of robot foundation models (RFMs), including VLAs~\cite{openvla,pi0,rt2}, world models~\cite{cosmos3,dreamzero,lingbot_va}, and video generation models~\cite{gr1,gr2}. This paradigm assumes that generalization emerges naturally once data and parameters are scaled sufficiently.

% However, deploying this paradigm in the open physical world exposes three fundamental challenges.
% \textbf{(1) The action-state space is continuous and unbounded.}
% Language can be discretized into a finite vocabulary, but robots operate in a continuous, high-dimensional state and action space, with visual noise orders of magnitude larger than textual noise; every action also shifts the data distribution for the next timestep. Training a policy by simply scaling up data collection is thus prohibitively expensive, and pure data scaling hits a hard wall.
% \textbf{(2) Predictive correlation does not transfer.}
% VLAs or WAMs are fundamentally correlational models: what they learn is ``execute this trajectory given this scene'' rather than ``this action changes the state in this way.'' Predictive structure is not causal structure, and this gap causes severe degradation under distribution shift---particularly sim-to-real---where a two-centimeter change in table height can cause outright failure.
% \textbf{(3) Consolidated knowledge cannot be updated by deployment experience.}
% The open world is irregular and continuously evolving, and cannot be exhausted by pretraining weights of any scale; yet once an existing RFM is deployed, its behavior is entirely determined by knowledge consolidated during pretraining, with no mechanism to absorb newly occurring interaction.


However, deploying this paradigm in the open physical world exposes three fundamental challenges.
\textbf{(1) The action-state space is continuous and unbounded:} robots operate in a continuous, high-dimensional state and action space, with visual noise orders of magnitude larger than textual noise, where every action also shifts the data distribution for the next timestep, making pure data scaling prohibitively expensive.
\textbf{(2) Predictive correlation does not transfer:} VLAs and WAMs are correlational models that learn to reproduce trajectories rather than model how actions cause state change; this gap produces severe degradation under distribution shift, particularly sim-to-real.
\textbf{(3) Consolidated knowledge cannot be updated by deployment experience:} the open world cannot be exhausted by pretraining weights of any scale, yet once deployed an RFM has no mechanism to absorb newly occurring interaction.



% Existing work each addresses one facet of these challenges but not all of them jointly: latent-action models~\cite{behaviorvla,alam,lapa} mitigate distribution shift through low-dimensional behavioral representations, but their representation spaces are fixed after pretraining and cannot expand from deployment interaction; memory-augmented methods~\cite{memoryvla,mem,dimwam} maintain observation history online, but what they store are visual or semantic features rather than the association between an action and the state change it induces, and this memory is cleared at the end of every episode; self-evolving methods~\cite{recap,vla_rl} and test-time training methods~\cite{robottt,wamttt} improve the policy from deployment experience, but the former rely on offline gradient retraining and the latter require gradient updates at inference time, so neither can accumulate cross-attempt experience under a gradient-free constraint. No framework yet accumulates deployment interaction experience across attempts and crystallizes that experience into an action-environment causal memory that guides subsequent decisions. To close this gap, we propose \textbf{Zeva}.



Existing work each addresses one facet of these challenges but not all jointly: latent-action models~\cite{behaviorvla,alam,lapa} mitigate distribution shift through low-dimensional behavioral representations fixed after pretraining; memory-augmented methods~\cite{memoryvla,mem,dimwam} maintain online observation history that stores visual or semantic features rather than action-induced state change, cleared at the end of every episode; self-evolving~\cite{recap,vla_rl} and test-time training methods~\cite{robottt,wamttt} improve the policy from deployment experience, but the former relies on offline gradient retraining too slow to inform the very next attempt, while the latter requires gradient updates during single-task inference and thus cannot accumulate experience across attempts. No framework yet accumulates deployment experience across attempts and crystallizes it into an action-environment causal memory that guides subsequent decisions. To close this gap, we propose \textbf{Zeva}.


% Zeva continuously extracts causal memory from the robot's own real interactions and uses this memory to condition every decision. The unbounded, continuous action-state space and the inability of predictive correlation to transfer together rule out pure data scaling---the robot must instead extract the causal relationship between actions and environmental change, trading causal structure for data efficiency and cross-distribution transfer. The open world's irregularity and continual evolution, which no pretraining weights can exhaust, further require the robot to self-evolve through ongoing interaction after deployment, rather than relying on a one-shot pretraining pass to cover every scenario. Both points converge on the same remedy: a \textbf{causal Interaction Memory} that is accumulated online from the robot's own interactions and retrieved at decision time---because it requires no gradient computation, this memory takes effect immediately within the time window between two attempts, allowing an embodied agent to keep scaling its capability after deployment without modifying any model weights.

Zeva's design follows two observations. The unbounded action-state space and the inability of predictive correlation to transfer rule out pure data scaling, requiring the robot to instead extract the causal relationship between actions and environmental change, trading causal structure for data efficiency and cross-distribution transfer; the open world's irregularity and continual evolution, which no pretraining can exhaust, further require the robot to self-evolve through post-deployment interaction rather than a one-shot pretraining pass. Both observations converge on a \textbf{Causal Interaction Memory} that is accumulated online from the robot's own interactions and retrieved at decision time. Since it requires no gradient computation, it takes effect within the time window between two attempts, letting an embodied agent keep scaling its capability after deployment without modifying any model weights.



% To realize Zeva, we decompose the construction and use of this memory into three stages. The \textbf{Causal Interaction Extraction} stage is carried out by Visual-Behavioral Dynamics (VBD): at every environment step, it records the action just executed and the visual state change it caused, and recursively accumulates these records into a continuously updated causal history state, which in turn yields a representation of the current task phase and of recent dynamics for later memory retrieval and action decision-making. The \textbf{Dual-timescale Interaction Memory} stage organizes these records at two timescales: a Brief Interaction Trace retains the most recent records within the current episode and is cleared on episode reset, while a Persistent Interaction Memory (PIM) accumulates continuously across episodes, controlling redundancy through similarity-based merging and consolidating the robot's interaction experience with the environment. The \textbf{Memory-Conditioned Policy} stage uses a Memory Context Encoder to fuse both memory streams together with task and phase information into a fixed-length sequence of clean semantic tokens, which are injected as conditioning into Cosmos3's~\cite{cosmos3} generation split without added diffusion noise and without contributing to the flow loss; at deployment, all model parameters remain frozen, and only the two memory streams are updated by interaction.



To realize Zeva, we decompose the memory construction and use into three stages. The \textbf{Causal Interaction Extraction} stage is carried out by Visual-Behavioral Dynamics (VBD): at every environment step it records the action just executed and the visual state change it caused, recursively accumulating these records into a Causal Interaction State that yields representations of the current task phase and recent interaction for memory retrieval and decision-making. The \textbf{Dual-timescale Interaction Memory} stage organizes these records at two timescales: a \textbf{Brief Interaction Trace} (BIT) retains the most recent records within the current attempt and is cleared at the next attempt, while a \textbf{Persistent Interaction Memory} (PIM) accumulates across attempts of the same episode with similarity-based merging. The \textbf{Memory-Conditioned Policy} stage uses a Memory Context Encoder to fuse both memory streams with task and phase information into fixed-length clean semantic tokens injected into Cosmos3's~\cite{cosmos3} generation split; at deployment, all model parameters remain frozen and only the two memory streams are updated by interaction.



We evaluate Zeva...
